Turbo-Aggregate: Breaking the Quadratic Aggregation Barrier in Secure Federated Learning

Federated learning is a distributed framework for training machine learning models over the data residing at mobile devices, while protecting the privacy of individual users. A major bottleneck in scaling federated learning to a large number of users is the overhead of secure model aggregation across many users. In particular, the overhead of the state-of-the-art protocols for secure model aggregation grows quadratically with the number of users. In this paper, we propose the first secure aggregation framework, named Turbo-Aggregate, that in a network with $N$ users achieves a secure aggregation overhead of $O(N\log{N})$, as opposed to $O(N^2)$, while tolerating up to a user dropout rate of $50\%$. Turbo-Aggregate employs a multi-group circular strategy for efficient model aggregation, and leverages additive secret sharing and novel coding techniques for injecting aggregation redundancy in order to handle user dropouts while guaranteeing user privacy. We experimentally demonstrate that Turbo-Aggregate achieves a total running time that grows almost linear in the number of users, and provides up to $40\times$ speedup over the state-of-the-art protocols with up to $N=200$ users. Our experiments also demonstrate the impact of model size and bandwidth on the performance of Turbo-Aggregate.

==> App_broader_impact.tex <==
% \textbf{Instruction:
% This section does not count towards the 8-page limit, and it should go before the references. It should include a statement about the foreseeable positive impact as well as potential risks and associated mitigations of the proposed research. We expect authors to write about two paragraphs, minimizing broad speculations. Authors can also declare that a broader impact statement is not applicable to their work, if they believe it to be the case. Reviewers will be asked to review papers on the basis of technical merit. Reviewers will also confirm whether the broader impact section is adequate, but this assessment will not affect the overall rating. However, reviewers will also have the option to flag a paper for ethical concerns, which may relate to the content of the broader impact section. If such concerns are shared by the Area Chair and Senior Area Chair, the paper will be sent for additional review to a pool of emergency reviewers with expertise in Machine Learning and Ethics, who will provide an assessment solely on the basis of ethical considerations. Program Chairs will then review each such case, aggregate all the feedback and make a final decision on the paper. We expect very few, if any, papers to need such further assessment. More information is available in the FAQ.}


The major societal benefit of our framework is facilitating privacy-aware distributed training at a very large scale. This can help application developers to provide better user experience by training  better, more accurate models, and at the same time protect the privacy of the individual users. 
Privacy protection is a growing societal concern due to the rapid increase in the volume and diversity of the data available from mobile devices. 
% As such, failure to protect the sensitive user information can have serious ethical and societal consequences. 
Federated learning is a promising framework for machine learning training in a distributed mobile environment, to protect the privacy of the data collected by individual mobile users from other users or the server who coordinates the training. Our protocol is the first protocol that can facilitate secure federated learning at a significantly low complexity, and hence future federated learning systems can benefit from our design principles to scale to a very large number of users. As a result, our framework can facilitate large-scale deployment of privacy-preserving distributed training protocols in real-world applications. 
% Moreover, our framework can be applied to peer-to-peer and decentralized communication setups,  
% As the proposed protocol enable more users to collaboratively train the model, users can obtain a high quality model service.
This can be a promising solution when the training dataset contains sensitive information such as genetic information, financial transactions, or geolocation information, as well as when data labelling is costly and can take a long time, such as data collected and labeled in medical fields. For example, one can train an accurate healthcare model to predict a potential disease, over the data available from the users of smartphones and wearable devices,  with their personal data measured from the health sensors of the device, while keeping the data private.  


A potential risk associated with our framework is that the private information of the users may be revealed if the number of colluding users is sufficiently large (larger than half of the total number of users participating in the protocol). 
In large-scale systems with more than tens of thousands of devices, for which the  federated learning systems are envisioned~\cite{bonawitz2019towards}, it is relatively unlikely that adversaries can control more than half of the participating users. However, this could still be a potential risk in small-scale systems. 
In addition, our focus was on honest but curious adversaries, i.e., the adversaries try to learn information about others but do not modify the protocol or inject false information into the datasets. Extending our framework to additional adversarial settings is an interesting future direction. 
% Another potential limitation is that the communication overhead of our protocol is higher than training protocols without privacy constraints, which can slow down training or cause delays if the channel quality is very poor. Finally, our protocol (and secure aggregation protocols in general) allows the server and the mobile users to learn the final  model. This may lead to inference attacks, where an adversary may try to extract information about individual users from the final trained model. Such scenarios may require additional protection for the datasets, such as introducing anonymity constraints. 
% via injecting intentional noise to the dataset or the local updates. 

% , such as using a noisy release mechanism as in  differential privacy, via injecting noise to the dataset or the local updates before the aggregation stage. 


% Federated learning has demonstrated that leveraging the information that is distributed over many mobile users can increase the training performance dramatically, while ensuring data privacy and locality. 
% Proposed protocol significantly reduces the computation and communication overhead of secure aggregation in Federated learning setting, which enables much better scalability with the number of users. As the proposed protocol enable more users to collaboratively train the model, users can obtain a high quality model service. 
% It can be more promising solution when the training dataset contain sensitive information such as genetic information, financial transactions, and geolocation information as well as when data labelling is costly and can take a long time, such as data collected and labeled in medical fields. For example, smartphone users can collaboratively train an accurate healthcare model to predict a potential disease with their personal data measured from the health sensors of the smartphone, while keeping the data private.  

% At the same time, this work may have some negative consequences because the private information can be revealed when the number of colluding users are larger than half of participating users. 
% However, as more than tens of thousands of devices are participating the federated learning~\cite{bonawitz2019towards}, it is prohibited that adversaries can control more than half of participating users. 
% In addition, our focus was on honest but curious adversaries, i.e., the adversaries try to learn information about others but do not inject false information into the protocol, for instance, via modifying their local datasets. The setup when adversaries can modify their local datasets to influence the global model has been studied in the literature in the context of non-secure federated learning. These frameworks often rely on comparing the distances between the local updates of the users, and excluding the outlier instances. Extending these frameworks to the secure federated learning paradigm is an interesting future direction, and requires additional challenges to be addressed, such as computing the distances between individual models of the users in a secure computation framework, without revealing the actual models.

==> App_generalizedTA.tex <==
The modified protocol follows the same steps in  Algorithm~\ref{Alg} except that the random mask $\mathbf{u}_i^{(l)}$ in~\eqref{eq:gen_SS} is generated by each user individually, instead of being generated by the server. At the end of the aggregation phase, the server learns  $\sum_{m\in[L]}\sum_{j\in\mathcal{U}_m}(\mathbf{x}^{(m)}_j+\mathbf{u}^{(m)}_j)$. 
    % , which corresponds to the aggregate of user models masked by the randomness added by the users.
    % instead of $\sum_{m\in[L]}\sum_{j\in\mathcal{U}_m}\mathbf{x}^{(m)}_j$. 
Simultaneously, the protocol executes an additional random partitioning strategy allocating $N$ users into $L$ groups with a group size of $N_{l}$. In this second partitioning, user $i$ in group $l'\in[L]$ secret shares ${\mathbf{u}}^{(l')}_i$ with the users in group $l'+1$, by generating and sending a secret share denoted by $[{\mathbf{u}}^{(l')}_i]_j$ to user $j$ in group $l'+1$. To do so, we utilize Shamir's  $\frac{N_{l}}{2}$-out-of-$N_l$ secret sharing~\cite{shamir1979share}. 
% with a  polynomial degree $\frac{N_{l}}{2}$ \cite{shamir1979share}. 
Let $\mathcal{U}^{'}_{l'}$ denote the surviving users in group $l'$ for the second partitioning. 
User $i$ in group $l'$ then aggregates the received secret shares $\sum_{j\in\mathcal{U}^{'}_{l'-1}}{\big[\mathbf{u}}^{(l'-1)}_j\big]_i$, which in turn is a secret share of  $\sum_{j\in\mathcal{U}^{'}_{l'-1}}{\mathbf{u}}^{(l'-1)}_j$, and sends the sum to the server. 
% User $i$ in group $l'$ then aggregates the received secret shares $\sum_{j\in\mathcal{U'}_{l'-1}}{\big[\mathbf{u}}^{(l'-1)}_j\big]_i$, which in turn is a secret share of  $\big[\sum_{j\in\mathcal{U'}_{l'-1}}{\mathbf{u}}^{(l'-1)}_j\big]_i$, where $\mathcal{U'}_{l'}$ denotes the surviving users in group $l'$, and sends the sum to the server.
Finally, the server reconstructs $\sum_{j\in\mathcal{U}^{'}_{l'}}{\mathbf{u}}^{(l')}_j$ for all $l'\in[L]$ and recovers the aggregate of the individual models of all surviving users by subtracting $\big\{ \sum_{j\in\mathcal{U}^{'}_{l'}}{\mathbf{u}}^{(l')}_j \big\}_{l'\in[L]}$ from the aggregate $\sum_{m\in[L]}\sum_{j\in\mathcal{U}_m}(\mathbf{x}^{(m)}_j+\mathbf{u}^{(m)}_j)$. 
% In this generalized version of {\name}, the privacy of any partial aggregation can be protected. 
In this generalized version of {\name}, the privacy of any partial aggregation, i.e., the aggregate of any subset of user models, can be protected as long as a  collusion between the server and the users does not reveal the aggregation of the random masks, $\sum_{j\in\mathcal{U}_{l}}{\mathbf{u}}^{(l)}_j$ in \eqref{eq:prop_partialsum} for any $l\in[L]$. 
Since there are at least $\frac{N}{2}$ unknown random masks generated by honest users and the server only knows $L=\frac{N}{N_l}$ equations, i.e., $\big\{ \sum_{j\in\mathcal{U}^{'}_{l}}{\mathbf{u}}^{(l)}_j \big\}_{l\in[L]}$,
the server cannot calculate $\sum_{j\in\mathcal{U}_{l}}{\mathbf{u}}^{(l)}_j$ for any $l\in[L]$. 
Therefore, a collusion between the server and users cannot reveal the partial aggregate as they cannot remove the random masks in~\eqref{eq:prop_partialsum}.
We now formally state the privacy guarantee, robustness guarantee, and  aggregation overhead of the generalized {\name} protocol in  Corollary~\ref{col:modifiedTA_achieve}.


\vspace{0.2cm}
\begin{corollary}~\label{col:modifiedTA_achieve}
Generalized {\name} simultaneously achieves 1), 2), and 3) from  Theorem~\ref{thm:TA_achieve}. In addition, it provides privacy guarantee for the partial aggregate of any subset of user models, against any collusion between the server and up to $T=(0.5-\epsilon)N$ users for any $\epsilon>0$, with probability approaching to $1$ as the number of users $N\rightarrow \infty$. 
% Generalized {\name} simultaneously achieves 1), 2), and 3) from  Theorem~\ref{thm:TA_achieve}. In addition, it provides privacy guarantee for the aggregate of any subset of user models, against any collusion between the server and up to $T=(0.5-\epsilon)N$ users for any $\epsilon>0$, with probability approaching to $1$ as the number of users $N\rightarrow \infty$. 
\end{corollary}
% \begin{proof*} \normalfont The proof of Corollary~\ref{col:modifiedTA_achieve} is presented in Appendix~\ref{app:proof_corollary}.
% \end{proof*}
% \noindent
\begin{proof}%[Corollary~\ref{col:modifiedTA_achieve}]
    The proof of Theorem~\ref{thm:TA_achieve} is presented in Appendix~\ref{app:proof_thm}.
\end{proof}

% \begin{remark} \normalfont
%     We note that the secure aggregation framework of \cite{bonawitz2017practical} can also be applied to a similar multi-group structure, by partitioning the network into multiple groups and applying the secure aggregation protocol from \cite{bonawitz2017practical} to each group. 
%     % The difference between this setup, i.e., \cite{bonawitz2017practical} applied to a multi-group structure, and our framework is that {\name} provides full privacy, i.e., server only learns the final aggregate of all groups (all $N$ users), whereas in the multi-group version of \cite{bonawitz2017practical}, the server would learn the aggregate model of each group.
%     The difference between this setup and our framework is that {\name} provides full privacy, i.e., server only learns the final aggregate of all groups, whereas in the multi-group version of \cite{bonawitz2017practical}, the server would learn the aggregate model of each group.
%     % Therefore, the two setups, i.e., \cite{bonawitz2017practical} applied to a multi-group structure vs. {\name}, are not comparable.
%     Therefore, these two setups are not comparable.
% \end{remark}
